LHAASO detection of very-high-energy gamma-ray emission surrounding PSR J0248+6021

We report the detection of an extended very-high-energy (VHE) gamma-ray source coincident with the location of middle-aged (62.4~\rm kyr) pulsar PSR J0248+6021, by using the LHAASO-WCDA data of live 796 days and LHAASO-KM2A data of live 1216 days. A significant excess of \gray induced showers is observed both by WCDA in energy bands of 1-25~\rm TeV and KM2A in energy bands of $>$ 25~\rm TeV with 7.3 $\sigma$ and 13.5 $\sigma$, respectively. The best-fit position derived through WCDA data is R.A. = 42.06$^\circ \pm$ 0.12$^\circ$ and Dec. = 60.24$^\circ \pm $ 0.13$^\circ$ with an extension of 0.69$^\circ\pm$0.15$^\circ$ and that of the KM2A data is R.A.= 42.29$^\circ \pm $ 0.13$^\circ$ and Dec. = 60.38$^\circ \pm$ 0.07$^\circ$ with an extension of 0.37$^\circ\pm$0.07$^\circ$. No clear extended multiwavelength counterpart of this LHAASO source has been found from the radio band to the GeV band. The most plausible explanation of the VHE \gray emission is the inverse Compton process of highly relativistic electrons and positrons injected by the pulsar. These electrons/positrons are hypothesized to be either confined within the pulsar wind nebula or to have already escaped into the interstellar medium, forming a pulsar halo.

==> AFFILIATIONS.tex <==
\twocolumn

\vspace*{0.5cm}
\noindent
$^{1}$ Key Laboratory of Particle Astrophyics \& Experimental Physics Division \& Computing Center, Institute of High Energy Physics, Chinese Academy of Sciences, 100049 Beijing, China\\
$^{2}$ University of Chinese Academy of Sciences, 100049 Beijing, China\\
$^{3}$ Tianfu Cosmic Ray Research Center, 610000 Chengdu, Sichuan,  China \\
$^{4}$ Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, 2 Dublin, Ireland \\
$^{5}$ Max-Planck-Institut for Nuclear Physics, P.O. Box 103980, 69029  Heidelberg, Germany\\
$^{7}$ State Key Laboratory of Particle Detection and Electronics, China\\
$^{8}$University of Science and Technology of China, 230026 Hefei, Anhui, China\\
$^{9}$ School of Astronomy and Space Science, Nanjing University, 210023 Nanjing, Jiangsu, China\\
$^{10}$ Center for Astrophysics, Guangzhou University, 510006 Guangzhou, Guangdong, China\\
$^{11}$ Hebei Normal University, 050024 Shijiazhuang, Hebei, China\\
$^{12}$ Key Laboratory of Dark Matter and Space Astronomy \& Key Laboratory of Radio Astronomy, Purple Mountain Observatory, \\Chinese Academy of Sciences, 210023 Nanjing, Jiangsu, China\\
$^{13}$ Tsung-Dao Lee Institute \& School of Physics and Astronomy, Shanghai Jiao Tong University, 200240 Shanghai, China\\
$^{14}$ Key Laboratory for Research in Galaxies and Cosmology, Shanghai Astronomical Observatory, \\ Chinese Academy of Sciences, 200030 Shanghai, China\\
$^{15}$ Key Laboratory of Cosmic Rays (Tibet University), Ministry of Education, 850000 Lhasa, Tibet, China\\
$^{16}$ National Astronomical Observatories, Chinese Academy of Sciences, 100101 Beijing, China\\
$^{17}$ School of Physics and Astronomy (Zhuhai) \& School of Physics (Guangzhou) \& Sino-French Institute of Nuclear Engineering and Technology (Zhuhai), Sun Yat-sen University, \\ 519000 Zhuhai \& 510275 Guangzhou, Guangdong, China \\
$^{18}$ School of Physics and Astronomy, Yunnan University, 650091 Kunming, Yunnan, China\\
$^{19}$ D\'epartement de Physique Nucl\'eaire et Corpusculaire, Facult\'e de Sciences, Universit\'e de Gen\`eve,\\ 24 Quai Ernest Ansermet, 1211 Geneva, Switzerland\\
$^{20}$ Institute of Frontier and Interdisciplinary Science, Shandong University, 266237 Qingdao, Shandong, China\\
$^{21}$ APC, Universit\'e Paris Cit\'e, CNRS/IN2P3, CEA/IRFU, Observatoire de Paris, 119 75205 Paris, France \\
$^{22}$ Department of Engineering Physics, Tsinghua University, 100084 Beijing, China \\
$^{23}$ School of Physics and Microelectronics, Zhengzhou University, 450001 Zhengzhou, Henan, China\\
$^{24}$ Yunnan Observatories, Chinese Academy of Sciences, 650216 Kunming, Yunnan, China\\
$^{25}$ College of Physics, Sichuan University, 610065 Chengdu, Sichuan, China\\
$^{26}$ Institute for Nuclear Research of Russian Academy of Sciences, 117312 Moscow, Russia \\
$^{27}$ Moscow Institute of Physics and Technology, 141700 Moscow, Russia\\
$^{28}$ School of Physics, Peking University, 100871 Beijing, China\\
$^{29}$ School of Physical Science and Technology, Guangxi University, 530004 Nanning, Guangxi, China\\
$^{30}$ Department of Physics, Faculty of Science, Mahidol University, Bangkok 10400, Thailand\\
$^{31}$ Center for Relativistic Astrophysics and High Energy Physics, School of Physics and Materials Science \& Institute of Space Science and Technology,\\ Nanchang University, 330031 Nanchang, Jiangxi, China\\
$^{32}$ National Space Science Center, Chinese Academy of Sciences, 100190 Beijing, China\\
